TutorTrace: A Dataset and Taxonomy for Classifying Learner Behavioral States during AI-Assisted Programming Education

AI programming tutors provide scalable support, yet lack the behavioral context human tutors rely on to adapt support to learners' needs. We present TutorTrace, a dataset and behavioral abstraction pipeline that makes learners' behavioral context visible and computable in real time from low-level IDE telemetry. Across four deployments in two introductory Python courses (N=480), TutorTrace captures approximately 180K telemetry events, 13,633 behavioral segments, and 27 continuously computed metrics. From this foundation, we derive a taxonomy of learner activity before the first AI query, between consecutive queries, and across the full session, enabling systems to respond not just to what learners say, but to what they have done leading up to the help-seeking moment. In a preliminary classroom evaluation, behavior-aware prompts were associated with a decrease in intervals between queries with no independent work from 50.0% to 20.7%. As an additional demonstration of downstream utility, we evaluate TutorTrace on two held-out prediction tasks: whether a learner will query within the next 60 seconds (AUROC=.726) and whether an upcoming query reflects guided or dependent help-seeking (AUROC=.717). Together, these findings show how behavioral context can enable adaptive AI tutoring at scale.

==> three-window_table.tex <==
\begin{table*}[!t]
\centering
\fontsize{8.0}{9.6}\selectfont
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.05}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\begin{tabular}{
  >{\raggedright\arraybackslash}p{1.3cm}
  >{\centering\arraybackslash}p{3.4cm}
  >{\raggedright\arraybackslash}p{2.0cm}
  R{0.85cm} R{0.6cm} R{0.55cm} R{0.5cm} R{0.5cm}
  >{\raggedright\arraybackslash}p{2.3cm}
}
\toprule

% ── WINDOW 1 ─────────────────────────────────────────────────
\multicolumn{9}{l}{%
  \rule{0pt}{10pt}%
  \textbf{Window 1 --- Before First Query}%
} \\
\midrule

\textbf{Profile}
  & \textbf{Example pre-query window}
  & \textbf{Description}
  & \textbf{N (\%)}
  & \textbf{Think}
  & \textbf{Runs}
  & \textbf{Err.}
  & \textbf{Pass}
  & \textbf{Intervention} \\
\midrule

Cold Start
  & \timeline{0.8800/thinkcolor, 0.1200/seekcolor}
  & First query.\ No prior attempt                                                
  & 31\,(20\%)
  & 72\,s
  & 0.0
  & 0.0
  & 97\%
  & Scaffold task entry.\ Offer pseudocode with blanks.\ End with a ``Try:'' starter. \\[3pt]

Oriented
  & \timeline{0.4200/thinkcolor, 0.2100/implcolor, 0.1400/thinkcolor, 0.0700/debugcolor, 0.0700/thinkcolor, 0.0900/seekcolor}
  & Made a genuine attempt, moderate code and effort before asking.
  & 100\,(66\%)
  & 98\,s
  & 1.2
  & 0.7
  & 92\%
  & Acknowledge the attempt.\ Unblock the specific error or gap. \\[3pt]

Struggling
  & \timeline{0.2000/thinkcolor, 0.1200/debugcolor, 0.1400/thinkcolor, 0.1600/debugcolor, 0.1000/thinkcolor, 0.1400/implcolor, 0.0600/thinkcolor, 0.0400/debugcolor, 0.0800/thinkcolor, 0.0600/seekcolor}
  & Extensive effort but no resolution with high runs, errors, edits before asking.
  & 21\,(14\%)
  & 165\,s
  & 4.2
  & 2.5
  & 67\%
  & Diagnose the misconception.\ Explain why the approach fails.\ Give a precise redirect. \\

\specialrule{1.0pt}{5pt}{3pt}

% ── WINDOW 2 ─────────────────────────────────────────────────
\multicolumn{9}{l}{%
  \rule{0pt}{10pt}%
  \textbf{Window 2 --- Between Queries}%
} \\
\midrule

\textbf{Profile}
  & \textbf{Example inter-query window}
  & \textbf{Description}
  & \textbf{N (\%)}
  & \textbf{Think}
  & \textbf{Runs}
  & \textbf{Err.}
  & \textbf{Pass}
  & \textbf{Intervention} \\
\midrule

Passive
  & \timeline{0.9000/thinkcolor, 0.1000/seekcolor}
  & Zero new effort since last AI response.\ Re-queries immediately.
  & 318\,(46\%)
  & 18\,s
  & 0.0
  & 0.0
  & 81\%
  & Try a different angle.\ Require student action before answering. \\[3pt]

Iterating
  & \timeline{0.3500/thinkcolor, 0.2200/implcolor, 0.1500/thinkcolor, 0.0800/implcolor, 0.0800/thinkcolor, 0.0700/debugcolor, 0.0500/seekcolor}
  & Light effort, one run, some edits, low error count.\ Steady progress.
  & 292\,(42\%)
  & 31\,s
  & 1.0
  & 0.5
  & 84\%
  & Validate the approach.\ Nudge toward the next step. \\[3pt]

Debugging
  & \timeline{0.1800/thinkcolor, 0.1200/implcolor, 0.1600/debugcolor, 0.1400/thinkcolor, 0.1800/debugcolor, 0.1000/thinkcolor, 0.0600/debugcolor, 0.0600/seekcolor}
  & Multiple runs and errors 
  & 56\,(8\%)
  & 57\,s
  & 3.7
  & 2.8
  & 79\%
  & Recognize the effort.\ Name the error.\ Escalate scaffolding. \\[3pt]

Spinning
  & \timeline{0.2800/thinkcolor, 0.2400/implcolor, 0.0800/thinkcolor, 0.1600/implcolor, 0.1000/thinkcolor, 0.0600/implcolor, 0.0800/thinkcolor, 0.0400/debugcolor, 0.0600/seekcolor}
  & High thinking and edits but barely tests.\ Writing without executing.
  & 22\,(3\%)
  & 149\,s
  & 1.8
  & 0.6
  & 50\%
  & Interrupt the loop.\ Direct to run code now.\ Explain why testing reveals the issue. \\

\specialrule{1.0pt}{5pt}{3pt}

% ── WINDOW 3 ─────────────────────────────────────────────────
\multicolumn{9}{l}{%
  \rule{0pt}{10pt}%
  \textbf{Window 3 --- Session-Wide Trajectory}%
} \\
\midrule

\textbf{Trajectory}
  & \textbf{Example session arc}
  & \textbf{Description}
  & \textbf{N (\%)}
  & \textbf{Avg\,Q}
  & \textbf{Q2\,Pa.}
  & \textbf{Comp.}
  &
  & \textbf{Intervention} \\
\midrule

Drifting
  & \timeline{0.1312/thinkcolor, 0.0111/debugcolor, 0.0129/thinkcolor, 0.0148/debugcolor, 0.0129/seekcolor, 0.0259/thinkcolor, 0.0111/seekcolor, 0.0148/thinkcolor, 0.0092/seekcolor, 0.0739/thinkcolor, 0.0518/debugcolor, 0.0314/thinkcolor, 0.0074/seekcolor, 0.0148/thinkcolor, 0.0111/seekcolor, 0.1238/thinkcolor, 0.0055/debugcolor, 0.2957/thinkcolor, 0.0314/debugcolor, 0.0129/seekcolor, 0.0222/thinkcolor, 0.0129/debugcolor, 0.0148/thinkcolor, 0.0296/debugcolor, 0.0092/thinkcolor, 0.0074/debugcolor}
  & Reaches for AI repeatedly.\ Passivity compounds with each query.
  & 133\,(79\%)
  & 7.5
  & 85\%
  & 85\%
  &
  & Interrupt passive re-querying.\ Require student action before next response. \\[3pt]

Persisting
  & \timeline{0.1449/thinkcolor, 0.0204/debugcolor, 0.0551/thinkcolor, 0.0041/debugcolor, 0.0245/thinkcolor, 0.0163/debugcolor, 0.0082/thinkcolor, 0.0204/debugcolor, 0.0224/seekcolor, 0.0469/thinkcolor, 0.0143/seekcolor, 0.0224/thinkcolor, 0.0020/debugcolor, 0.0245/thinkcolor, 0.0592/debugcolor, 0.0347/thinkcolor, 0.0449/seekcolor, 0.0857/thinkcolor, 0.0939/debugcolor, 0.0469/thinkcolor, 0.0245/debugcolor, 0.0224/thinkcolor, 0.0020/debugcolor, 0.0878/thinkcolor, 0.0714/debugcolor}
  & Works through extended debug loops independently.\ Rarely asks.
  & 22\,(13\%)
  & 1.6
  & 63\%
  & 86\%
  &
  & Recognize independent effort.\ Unblock the specific error. \\[3pt]

Bypassing
  & \timeline{0.2132/thinkcolor, 0.0251/seekcolor, 0.0878/thinkcolor, 0.0157/implcolor, 0.0219/thinkcolor, 0.1411/implcolor, 0.0251/thinkcolor, 0.0439/implcolor, 0.0251/thinkcolor, 0.0690/implcolor, 0.0219/thinkcolor, 0.0564/implcolor, 0.0408/thinkcolor, 0.0690/implcolor, 0.0219/thinkcolor, 0.0282/implcolor, 0.0188/thinkcolor, 0.0752/implcolor}
  & Writes code but skips testing before asking.
  & 11\,(7\%)
  & 0.8
  & 81\%
  & 91\%
  &
  & Direct to test existing code before explaining further. \\

\midrule

% ── LEGEND ───────────────────────────────────────────────────
\multicolumn{9}{c}{%
  \tikz[baseline=-0.3ex]{\fill[thinkcolor] (0,0) rectangle (0.28cm,0.17cm);}~Thinking\quad
  \tikz[baseline=-0.3ex]{\fill[implcolor]  (0,0) rectangle (0.28cm,0.17cm);}~Implementing\quad
  \tikz[baseline=-0.3ex]{\fill[debugcolor] (0,0) rectangle (0.28cm,0.17cm);}~Debugging\quad
  \tikz[baseline=-0.3ex]{\fill[seekcolor]  (0,0) rectangle (0.28cm,0.17cm);}~Seeking Help%
} \\

\bottomrule
\end{tabular}

\caption{The \sys{} three-window behavioral taxonomy. Each window captures a
distinct moment in the help-seeking cycle, characterized by different behavioral
signals and requiring different intervention strategies.}
\label{tab:taxonomy-unified}

\end{table*}
